ByTheWay: Boost Your Text-to-Video Generation Model to Higher Quality in a Training-free Way

The text-to-video (T2V) generation models, offering convenient visual creation, have recently garnered increasing attention. Despite their substantial potential, the generated videos may present artifacts, including structural implausibility, temporal inconsistency, and a lack of motion, often resulting in near-static video. In this work, we have identified a correlation between the disparity of temporal attention maps across different blocks and the occurrence of temporal inconsistencies. Additionally, we have observed that the energy contained within the temporal attention maps is directly related to the magnitude of motion amplitude in the generated videos. Based on these observations, we present ByTheWay, a training-free method to improve the quality of text-to-video generation without introducing additional parameters, augmenting memory or sampling time. Specifically, ByTheWay is composed of two principal components: 1) Temporal Self-Guidance improves the structural plausibility and temporal consistency of generated videos by reducing the disparity between the temporal attention maps across various decoder blocks. 2) Fourier-based Motion Enhancement enhances the magnitude and richness of motion by amplifying the energy of the map. Extensive experiments demonstrate that ByTheWay significantly improves the quality of text-to-video generation with negligible additional cost.

==> table/quantitative.tex <==
\begin{table*}[]
\resizebox{\linewidth}{10mm}{
\begin{tabular}{lccccccccc}
\toprule[1.5pt]
\multirow{2}{*}{Evaluation Metric} & \multicolumn{1}{c}{(a) User Study} & \multicolumn{6}{c}{(b) VBench~\citep{huang2023vbench} Metrics} & \multicolumn{2}{c}{(c) MLLM Assessment} \\ \cmidrule(r){2-2} \cmidrule(r){3-8} \cmidrule(r){9-10}
   & Video Quality~ & Subject Consistency~  & Background Consistency~ & Motion Smoothness~ & Dynamic Degree~  & Aesthetic Quality~ & Imaging Quality~ & Structure Rationality~  & Motion Consistency~  \\ \midrule[0.5pt]
AnimateDiff~\citep{guo2023animatediff}    & 25.42\%    & 0.9738 & 0.9717 & 0.9774    & 0.1373 & 0.6571 & 0.7515    & 41.94\% &  34.62\% \\
\rowcolor{gray!10}\textbf{AnimateDiff + \method}           & \textbf{74.58\%}    & \textbf{0.9744} & \textbf{0.9725} & \textbf{0.9786}    & \textbf{0.2941} & \textbf{0.6609} & \textbf{0.7553}    & \textbf{58.06\%} & \textbf{65.38\%}  \\
\addlinespace
VideoCrafter2~\citep{chen2024videocrafter2} & 30.54\%    & 0.9840 & 0.9891 & 0.9849  & 0.1586 & 0.6477 & 0.6075    & 18.48\% & 39.60\%   \\
\rowcolor{gray!10}\textbf{VideoCrafter2 + \method}           & \textbf{69.46\%}    & \textbf{0.9852} & \textbf{0.9896} & \textbf{0.9863}  &  \textbf{0.5547} & \textbf{0.6498} & \textbf{0.6338}    & \textbf{81.52\%} & \textbf{60.40\%}  \\ 
 \bottomrule[1.5pt]
\end{tabular}
}
\centering
\vspace{-1em}
\caption{\textbf{Quantitative results of \method.}
\method-enhanced backbones outperform baseline T2V backbones in numerous strong metrics, including our user study, all VBench~\citep{huang2023vbench} metrics on customized video evaluation and a MLLM assessment utilizing GPT-4o~\citep{achiam2023gpt4}.
}
\label{tab:quant}
\end{table*}
